5GLoR: 5G LAN Orchestration for enterprise IoT applications

5G-LAN is an enterprise local area network (LAN) that leverages 5G technology for wireless connectivity instead of WiFi. 5G technology is unique: it uses network slicing to distinguish customers in the same traffic class using new QoS technologies in the RF domain. This unique ability is not supported by most enterprise LANs, which rely primarily on DiffServ-like technologies that distinguish among traffic classes rather than customers. We first show that this mismatch in QoS between the 5G network and the LAN affects the accuracy of insights from the LAN-resident analytics applications. We systematically analyze the root causes of the QoS mismatch and propose a first-of-a-kind 5G-LAN orchestrator (5GLoR). 5GLoR is a middleware that applications can use to preserve the QoS of their 5G data streams through the enterprise LAN. 5GLoR periodically analyzes the status of the queues, provides suitable DSCP identifiers to the application, and installs relevant switch re-write rules (to change DSCP identifiers between switches) to continuously preserve the QoS of the 5G data through the LAN. 5GLoR improves the RTP frame level delay and inter-frame delay by 212\% and 122\%, respectively, for the WebRTC application. Additionally, with 5GLoR, the accuracy of two example applications (face detection and recognition) improved by 33\%, while the latency was reduced by about 25\%. Our experiments show that the performance (accuracy and latency) of applications on a 5G-LAN performs well with the proposed 5GLoR compared to the same applications on MEC. This is significant because 5G-LAN offers an order of magnitude more computing, networking, and storage resources to the applications than the resource-constrained MEC, and mature enterprise technologies can be used to deploy, manage, and update IoT applications.

==> background.tex <==
% A network slice is a resource pipeline for the application with a specific guarantee of isolation and QoS. The resources could be virtual or dedicated physical resources. This network slice helps support multiple applications with a diverse set of requirements. The 5G endorses the creation of such network slices that begin in the RAN and end at the 5G core. The network slice is identified using a $32-$bit number called Single Network Slice Selection Assistance Information (S-NSSAI), supporting the creation of $2^{24}$ slices. Eight bits allocation for the slice service types (SST) of slices, supporting 256 different slices in 5G and 24 bits for the Slice Differentiator (SD) supporting $2^{24}$ differentiator for each service type. 
  
% The 5G supports five different levels of isolation. Level 0/1/2 offers the sharing of resource blocks (RB) within RAN and tries to achieve the QoS guarantee based on priority. Level 3 has partially reserved RB and shares a specific RB in dynamic ways, and these slices have higher priorities than the previous. Level 4 has dedicated frequency channels for the RAN slice creation and has the highest priority.  


% When we need to support the applications with a diverse set of requirements, the 5G RAN slice can be used. As these applications need computing or storage, they must utilize the enterprise LANs to connect to the computing devices. Consider the figure \ref{fig:Context} where the surveillance camera is streaming over a 5G RAN slice or the thermal screening application that needs computing devices in the enterprise LAN. As we see in the same figure for one single application it might utilize single/multiple devices on the LAN. Or multiple slices in RAN can use one single device on the LAN. Creating a many to many relationship for flows from RAN to LAN. 

% The enterprise LANs are shared and built on the best effort ideology. So how would one support applications that use the 5G RAN slice with computing devices on the shared enterprise LAN? 
% In the LAN world, the class of service is the construct that supports the specific guarantee of QoS. Broadly the traffic classes are video, audio, real-time video, voice over IP (VoIP), and best effort traffic. These classes can ensure a certain level of guarantee of services. For example, the video traffic has 3\% dedicated resources on an outgoing interface. If the link capacity is 1Gbps, then video traffic will get a dedicated resource of 30 Mbps. This can only guarantee 30Mbps for all the video traffic. If the traffic is more than 30 Mbps, it needs to use the best effort resource where the guarantee is not promised, especially in the case of congested environments. The figure \ref{fig:ranlan} shows such a demonstration where the guarantee is broken when the interface is congested. Hence for complete RAN to LAN translation for the E2E slice support, there is a need for an 5GLoR or hypervisor that ensures the QoS guarantee using this class of service construct in the enterprise LAN. 

==> futurework.tex <==
\section{Discussion}
Our current system is built for a single IoT application. The number of RAN flows coming in with GBR requirements is smaller than the total available hardware queues. We can extend the 5GLoR for multi-tenant applications, where the number of RAN flows will be significantly more significant than the total available queues. This breaks the feasibility easily. we plan to extend our solution by adding proxy paths in LAN or exploring multipath capabilities of the LAN. The machine learning algorithms will be used to monitor the LAN flows and switches to avoid the complexities of increased RAN flows. 

% monitors the number of flows that provides equal share when congestion occurs. If the minimum share is below the maximum request of the RAN flows, we declare the queue as infeasible. We want to extend this model, where we can predict the increased rate of the total number of flows and queue occupation using linear regression or machine learning models, this will prevent in-feasibility before it occurs. We will also extend the work for down-link, where control is from application to the RAN.
